A Central Limit Theorem for Algorithmic Estimator of Saddle Point

In this work, we study the asymptotic randomness of an algorithmic estimator of the saddle point of a globally convex-concave and locally strongly-convex strongly-concave objective. Specifically, we show that the averaged iterates of a Stochastic Extra-Gradient (SEG) method for a Saddle Point Problem (SPP) converges almost surely to the saddle point and follows a Central Limit Theorem (CLT) with optimal covariance under martingale-difference noise and the state(decision)-dependent Markov noise. To ensure the stability of the algorithm dynamics under the state-dependent Markov noise, we propose a variant of SEG with truncated varying sets. Interestingly, we show that a state-dependent Markovian data sequence can cause Stochastic Gradient Descent Ascent (SGDA) to diverge even if the target objective is strongly-convex strongly-concave. The main novelty of this work is establishing a CLT for SEG for a stochastic SPP, especially under sate-dependent Markov noise. This is the first step towards online inference of SPP with numerous potential applications including games, robust strategic classification, and reinforcement learning. We illustrate our results through numerical experiments.

==> rebuttal.tex <==
\section{Global Response}
We would like to clarify upfront about the novelty of our results and the motivation of adopting the stochastic extra gradient (SEG) algorithm.
We note that the previous generic results in the stochastic averaging (SA) literature do not apply to the saddle point optimization problems and that using SEG is essential in obtaining a central limit theorem (CLT) with $\sqrt{n}$ rate, in particular in the state-dependent Markovian noise setting.
Specifically, Stochastic Gradient Descent Ascent (SGDA), which is the forward time-stepping algorithm considered in the existing SA literature, the iterates may not even converge with state-dependent Markovian noise.

We thank the reviewers for pointing us to the references. We have discussed them in more depth in individual responses and provide the example here that sets our work apart from them.

**SGDA  vs SEG in the state-dependent Markovian noise setting**

Let $$f(x,y)=x^\top y+0.5 \|x\|_2^2-0.5 \|y\|_2^2,$$ and $z\coloneqq (x,y)$. The saddle-point is $z^*=(0,0)$. 

Then $H(z_k)=[(y_k+x_k)^\top\quad (y_k-x_k)^\top]^\top$. Let the state-dependent noise in $H(z_{k-1},w_k)$ is 
$$\xi(z_{k-1},w_k)=[(x_{k-1}+{\nu_{1,k}})^\top\quad (y_{k-1}+{\nu_{2,k}})^\top]^\top$$ 
where ${\nu_{1,k}}\sim N(0,\sigma^2 I_d)$, ${\nu_{2,k}}\sim N(0,\sigma^2 I_d)$, ${\nu_{1,k}}$ and ${\nu_{2,k}}$ are independent of each other and filtration $\mathcal{F}_{k-1}$, and $\{\nu_{1,k}\}_k$ and $\{\nu_{2,k}\}_k$ are i.i.d sequence. 

**Verification of Assumption 6.1** Set $\mathcal{V}(w_k)=1+\|\nu_{1,k}\|_2^2+\|\nu_{2,k}\|_2^2$. For any fixed $z_k=z$, $\xi(z,w_k)$ is i.i.d Gaussian random variable. So it clearly satisfies the drift condition (Condition 1 of Assumption 6.1). It is easy to see that when $z$ belongs to a compact set, Condition 2 of Assumption 6.1 is true.  Since the transition kernel depends linearly on $z$, Condition 3 of Assumption 6.1 (Lipschitz continuity of the transition kernel) holds. 

Then, $$H(z_{k-1},w_k)=H(z_{k-1})-\xi({z_{k-1},w_k})=[(y_{k-1}-{\nu_{1,k}})^\top  \quad (-x_{k-1}-{\nu_{2,k}})^\top]^\top .$$ 
Then the SGDA update, which is classical SA algorithm, is given by, 
$$z_k=z_{k-1}-\eta_k[(y_{k-1}-{\nu_{1,k}})^\top  \quad (-x_{k-1}-{\nu_{2,k}})^\top]^\top .$$ SGDA leads to the following dynamics. 
\begin{align*}
    &E[\|x_k\|_2^2|\mathcal{F}_{k-1}]\\
    =&\|x_{k-1}\|_2^2-2\eta_k x_{k-1}^\top (y_{k-1}-E[\nu_{1,k}|\mathcal{F}_{k-1}])+\eta_{k}^2(\|y_{k-1}\|_2^2-2y_{k-1}^\top E[\nu_{1,k}|\mathcal{F}_{k-1}]+E[\|\nu_{1,k}\|_2^2|\mathcal{F}_{k-1}])\\
    =&\|x_{k-1}\|_2^2-2\eta_k x_{k-1}^\top y_{k-1}+\eta_{k}^2(\|y_{k-1}\|_2^2+d\sigma^2).
\end{align*}
Similarly, 
\begin{align*}
    E[\|y_k\|_2^2|\mathcal{F}_{k-1}]
    =E[\|y_{k-1}\|_2^2]+2\eta_k y_{k-1}^\top x_{k-1}+\eta_{k}^2(\|x_{k-1}\|_2^2+d\sigma^2).
\end{align*}
**Combining, one gets, 
\begin{align*}
    E[\|x_k\|_2^2+\|y_k\|_2^2|\mathcal{F}_{k-1}]=(1+\eta_k^2)(\|x_{k-1}\|_2^2+\|y_{k-1}\|_2^2)+2d\eta_k^2\sigma^2
\end{align*}

This clearly shows the problem with SGDA dynamics. We provide a comparison of the performance of SGDA and SEG in our global response pdf. We plot $\|\sqrt{n}\bar{x}_n\|_2^2+\|\sqrt{n}\bar{y}_n\|_2^2$. The difference between the asymptotic rates of SEG and SGDA is clear. **



\iffalse
Then,
\begin{align*}
    E[\|x_k\|_2^2]
    =E[\|x_{k-1}\|_2^2]-2E[\eta_k x_{k-1}^\top y_{k-1}]+\eta_{k}^2(E[\|y_{k-1}\|_2^2]+d\sigma^2).
\end{align*}

\begin{align*}
    E[\|x_k\|_2^2+\|y_k\|_2^2]=&(1+\eta_k^2)E[\|x_{k-1}\|_2^2+\|y_{k-1}\|_2^2]+2d\eta_k^2\sigma^2\\
    =&\textstyle\prod_{i=1}^k(1+\eta_i^2)(\|x_{0}\|_2^2+\|y_{0}\|_2^2)+2d\sigma^2(\eta_k^2+\sum_{i=1}^{k-1}\prod_{j=i+1}^{k}(1+\eta_j^2)\eta_i^2)
\end{align*}
Now, by Robbins and Siegmund theorem [1], one can only guarantee that , $\|x_k\|_2^2+\|y_k\|_2^2$
[1] Anbar, Dan. "An application of a theorem of Robbins and Siegmund." The Annals of Statistics (1976): 1018-1021. \url{https://www.jstor.org/stable/2958641?seq=1#metadata_info_tab_contents}
\fi




\newpage
%\section{Rebuttal}


\textbf{Reviewer uWYr}\\

{\bfseries To me, the main weakness of the paper is somehow limited novelty. There exist a lot of both asymptotic and non-asymptotic results around CLT for SA, in particular, there is a general work of [Fort, 2015], which the authors missed in the literature review, and which suggests a very general framework for obtaining CLT for the Polyak-Ruppert averaged SA. Moreover, there are deep non-asymptotic results of Berry-Esseen type, with tight dimension dependence, e.g. [Q. Shao, 2022]. Thus I believe that at least the first part of the submission (related to the martingale-difference noise) has limited novelty as compared to the literature, even despite the fact that there is no ready-to-use result for the saddle point problems with SEG. I believe that the proof can be easily obtained following the [Fort, 2015] setup.

Also, the asymptotic nature of the results is a significant restriction. The paper would be much stronger if the non-asymptotic error bounds would be provided.

References:

    Fort, G. (2015). Central limit theorems for stochastic approximation with controlled Markov chain dynamics. ESAIM: Probability and Statistics, 19, 60-80.
    Shao, Q. M., \& Zhang, Z. S. (2022). Berry–Esseen bounds for multivariate nonlinear statistics with applications to M-estimators and stochastic gradient descent algorithms. Bernoulli, 28(3), 1548-1576.}

    Thank you for the feedback. 

1. Fort, G. (2015) is indeed relevant to our work but there are significant differences between Fort, G. (2015) and our work. Here is the main difference between our work and Fort, G. (2015).

a) **Fort, G. (2015) studies classical Stochastic Approximation (SA) which may not even converge when the goal is to find a saddle point and the noise is state-dependent Markovian**

SEG is an approximation of a stochastic Proximal Point (PP) method [Proposition 2, 1] given by $$z_{k+1}=z_k-\eta_{k+1}H(z_{k+1},w_{k+1})$$ whereas Fort, G. (2015) studies classical Stochastic Approximation (SA) with the update $$z_{k+1}=z_k-\eta_{k+1}H(z_{k},w_{k+1})$$ which is also known as Stochastic Gradient Descent Ascent (SGDA). They are fundamentally different. It is well known that PP is more stable than SA [2 and the references therein]. In fact, in the state-dependent Markovian noise setting, SGDA may not even converge. Please see our **Global Response** for a fully worked out example and experiment results.  

Apart from this main fundamental difference, our work differs from that of Fort, G. (2015) in the following aspects as well. 

In the state-dependent Markovian noise setting:

b) Fort, G. (2015) assumes that only finite number of truncations are needed (Assumption A1). On the contrary, instead of assuming this, we explicitly prove this in Theorem 6.1 and the proof is quite non-trivial. 

c) Fort, G. (2015) assumes $H$ to be bounded which clearly fails in the strongly-convex strongly-concave case. 

d) Fort, G. (2015) only establishes the CLT for the iterates (not for the averaged iterates, Section 4, Proposition 4.1) of SA which does not achieve the optimal covariance. 

2. We agree that extending ther non-asymptotic results of Shao, Q. M., \& Zhang, Z. S. (2022) in the state-dependent Markovian noise setting and Saddle Point problems will be useful indeed. 

Given our results on asymptotic uncertainty of SEG for saddle point optimization are novel and the analysis is quite involved, we defer the non-asymptotic bounds for future work. 

Minor misprints and issues:

1. The constant $C$ depends on the Is the constant 

appearing in the stepsize instance dependent? If yes, please indicate its dependence on the problem-specific constants.
$C$ can be any positive constant. For constant step-size SEG, $\eta<1/C_1$ where $C_1=(4\mu+\sqrt{2}L_G)$ [3] is required. But since we are using polynomially decreasing step-size $\eta_k$ will be smaller than $1/C_1$ after $(2CC_1)^{1/a}$ iterates. Since the analysis is asymptotic, the results remain unchanged. 

2,4,5,6,7. Thanks for pointing these out. We will fix these issues. 

3. I suggest adding a sentence explaining what is the asymptotic optimality after Theorem~5.2;

We will add it.  


[1] Aryan Mokhtari, Asuman Ozdaglar, and Sarath Pattathil. A unified analysis of extra-gradient and optimistic gradient methods for saddle point problems: Proximal point approach. In International Conference on Artificial Intelligence and Statistics, pages 1497–1507. PMLR, 2020.\url{https://proceedings.mlr.press/v108/mokhtari20a.html}

[2] Bertsekas, Dimitri P. "Incremental proximal methods for large scale convex optimization." Mathematical programming 129, no. 2 (2011): 163-195.\url{https://www.mit.edu/~dimitrib/Incremental_Survey_LIDS.pdf}

[3] Gorbunov, Eduard, Hugo Berard, Gauthier Gidel, and Nicolas Loizou. "Stochastic extragradient: General analysis and improved rates." In International Conference on Artificial Intelligence and Statistics, pp. 7865-7901. PMLR, 2022.

%[3] Daskalakis, Constantinos, Andrew Ilyas, Vasilis Syrgkanis, and Haoyang Zeng. "Training gans with optimism." arXiv preprint arXiv:1711.00141 (2017).\url{https://arxiv.org/abs/1711.00141}


\textbf{Reviewer LoBv}

Q1. \textbf{Compared with stochastic minimization problems, what is the main difficulty of online inference for SPPs?}

Q2. \textbf{I do not understand why to adopt SEG for a strongly-convex strongly-concave objective. In such a case, the gradient field
is strongly monotone. Then stochastic gradient descent ascent (SGDA) could also converge at the rate. What is the advantage of SEG over SGDA for a strongly-convex strongly-concave objective?}

Q3. \textbf{The authors say that SEG is an approximation of the proximal point method in line 43. However, SEG (in Algorithm 1) can also be viewed as SGDA plus a correction term . And from the analysis in line 196, this correction term is negligible in the asymptotic sense. So I guess SGDA also enjoys the same properties of SEG in this paper. Then we come back to Question 1. And maybe it is more appropriate to view SEG as a variant of SGDA.}

Q1,2,3: We combine our replies to Q 1, 2, and 3 in the following answer. We first point out that **SEG is an approximation of proximal point update [Theorem 1 of 2, Prop. 2 of 4] whereas SGDA is classical SA. This is a crucial difference and this is why SEG converges in convex-concave problems but SGDA may not.** This also emphasizes the fact that stochastic minimization (where proximal point method and SA both converge) and stochastic saddle point problems are fundamentally different. 

**Even though we consider strongly-convex strongly-concave objective function, because of the state-dependence of the noise, SGDA may not converge. Please see our Global Response for a fully worked out example of this behavior.** 


\textbf{In equations (6) and (7), the two noisy observations are evaluated at the same sample. However, in the online setting, this may be invalid. If (6) and (7) use two different samples, do the results of this paper still hold?}

Note that using the same sample to evaluate the updates of SEG is possible in most machine learning applications like bi-linear games, generative adversarial networks, and adversarial training [1]. In fact there are examples where the SEG iteration persistently diverges when using independent samples [1]. Intuitively, this happens because with independent samples, SEG is no longer an approximation of proximal point method and hence can diverge. For detailed explanation see [Sec. 1 of 1, Sec. 2 of 2, Sec. 1.1 of 3]. 

\textbf{Why does vanish in the equation below line 195?}
This is indeed a typo. The term $T_2$ should be $\frac{1}{\sqrt{k}}\sum_{i=1}^k\sum_{j=1}^{i}\eta_jY_j^i(H(z_{j-1/2},w_{j})-H(z_{j-1},w_{j}))$. Although this does not change our proof steps and bound on the term $T_2$. Specifically, using Assumption~4.2, and Lemma~A.2, we still get,
\begin{align*}
\norm{T_2}_2^2
    =&\norm{\frac{1}{\sqrt{k}}\sum_{i=1}^k\sum_{j=1}^{i}\eta_jY_j^i(H(z_{j-1/2},w_j)-H(z_{j-1},w_j))}_2^2\\
    = &\norm{\frac{1}{\sqrt{k}}\sum_{j=1}^k\sum_{i=j}^{k}\eta_jY_j^i(H(z_{j-1/2},w_j)-H(z_{j-1},w_j))}_2^2\\
    \leq  &\frac{1}{k}\left(\sum_{j=1}^k\eta_j\norm{\sum_{i=j}^{k}Y_j^i}_2\norm{H(z_{j-1/2},w_j)-H(z_{j-1},w_j)}_2\right)^2\\
     \leq &\frac1k\left(\sum_{j=1}^kL_G\norm{z_{j-1/2}-z_{j-1}}_2\right)^2\\
     \leq &\frac1k\left(\sum_{j=1}^kL_G\eta_j\norm{H(z_{j-1},w_j)}_2\right)^2.
\end{align*}
\textbf{Assumption 6.1 is pretty obscure. Could the authors provide some examples satisfying this assumption?}

Q6. Section 3 presents the example illustrating SPP with state-dependent Markov noise. See line 305-313 in Section 7 where we show, with specific numbers, that Assumption 6.1 holds for the example in Section 3. 

Intuitively, 

i) Condition 1 of Assumption 6.1, is a drift condition which ensures that for fixed $z$, the Markovian data is $\mathcal{V}$-uniformly ergodic.

ii) Condition 2 states that within a compact set $z\in \mathcal{Z}'$, the gradient norm is is allowed to grow as fast as $C\mathcal{V}(w)$.

iii) Condition 3 imposes a regularity condition to control the change of the transition kernel $P_z$ with respect to $z$. In other words, it assumes $P_z$ is $V(w)$-Lipschitz continuous in the compact set $\mathcal{Z}'$.

Besides example 3, as we state in Remark 2, Assumption 6.1 holds for State-dependent Markov noise across various applications: strategic classification with adaptive best response [LW22]; policy-gradient [KMMW19], and actor-critic algorithm in reinforcement learning [WZXG20]; MLE with missing data [Lia10].

[1] Li, Chris Junchi, Yaodong Yu, Nicolas Loizou, Gauthier Gidel, Yi Ma, Nicolas Le Roux, and Michael Jordan. "On the convergence of stochastic extragradient for bilinear games using restarted iteration averaging." In International Conference on Artificial Intelligence and Statistics, pp. 9793-9826. PMLR, 2022.

[2] Mishchenko, Konstantin, Dmitry Kovalev, Egor Shulgin, Peter Richtárik, and Yura Malitsky. "Revisiting stochastic extragradient." In International Conference on Artificial Intelligence and Statistics, pp. 4573-4582. PMLR, 2020.

[3] Gorbunov, Eduard, Hugo Berard, Gauthier Gidel, and Nicolas Loizou. "Stochastic extragradient: General analysis and improved rates." In International Conference on Artificial Intelligence and Statistics, pp. 7865-7901. PMLR, 2022.

[4] Aryan Mokhtari, Asuman Ozdaglar, and Sarath Pattathil. A unified analysis of extra-gradient and optimistic gradient methods for saddle point problems: Proximal point approach. In International Conference on Artificial Intelligence and Statistics, pages 1497–1507. PMLR, 2020.

[5] Daskalakis, Constantinos, Andrew Ilyas, Vasilis Syrgkanis, and Haoyang Zeng. "Training gans with optimism." arXiv preprint arXiv:1711.00141 (2017).

**2nd response**

**\textbf{In the example of Global Response, $H(z_{k-1},w_k)$ can be decomposed as...plus the martingale different noise. The first term is just the gradient field of the function $x^\top y$. Could I interpret this as follows: If we want to eliminate the dependence of noise on the state, the objective should be changed?}**

In this particular and simple example, yes. 
%We wanted to highlight the difference between SEG and SGDA in a simple case. 
For simplicity, we have chosen $\xi(z_{k-1},w_k)$ such that it is decomposable into two components - one involving only $z_{k-1}$ and another dependent on $\iid$ noise sequence $\nu_{1,k}$ and $\nu_{2,k}$. 
% But note that, under Assumption~6.1, $\{\nu_{1,k}\}_k$ and $\{\nu_{2,k}\}_k$ can be Markovian too. 
In general, $\xi(z_{k-1},w_k)$ is not necessarily separable in terms of $z_{k-1}$ and $w_k$. 
In those cases, it is not possible to get a simple decomposition into a modified objective and a simple noise. Furthermore, Assumption 6.1 allows the $z$ dependence of $P_z$ to change throughout the dynamics leading to more complex dynamics than we present in the global response. 

**\textbf{...which is a strongly-concave-strongly-convex function. .  Does this imply that SEG could converge even when applied to such a function? Or which step went wrong?}**

In the case where the objective function $f$ becomes strongly-concave-strongly-convex, it does not even have a saddle point. So SEG can't converge. Recall that $(\theta^*,\mu^*)$ is defined as, 
\begin{align*}
    (\theta^*,\mu^*)\coloneqq\underset{\t\in\mathbb{R}^{d_{\t}}}{\argmin}~\underset{\m\in\mathbb{R}^{d_{\m}}}{\argmax}~\expec{F(\t,\m,w)}{}=\underset{\t}{\argmin}~\underset{\m}{\argmax}~f(\t,\m)
\end{align*}

If there is no such point then the problem itself is ill-defined.

We thank you for bringing this up. Your question actually makes us realize that we just need the strong-convexity strong-concavity to hold not globally but only in an arbitrarily small neighborhood $\mathcal{N}$ around $z^*$. Indeed, our proof really depends on the fact that the matrix $Q^*$ which is defined at $z^*$, is Hurwitz and satisfies Assumption 4.3 in $\mathcal{N}$. So if Assumption 4.1 is modified to say that $f(\theta,\mu)$ is strongly-convex strongly-concave only in an arbitrarily small neighborhood $\mathcal{N}$ around $z^*$, our proof and results hold as it is. 

Say $\mathcal{N}$ is given by $||z-z^*||\leq r$. Consider the following setup similar to the global example but with a little modification in the noise. 

Let $$f(x,y)=x^\top y+0.5 \|x\|_2^2-0.5 \|y\|_2^2,$$ and $z\coloneqq (x,y)$. The saddle-point is $z^*=(0,0)$. 

Then $H(z_k)=[(y_k+x_k)^\top\quad (y_k-x_k)^\top]^\top$. Let the state-dependent noise in $H(z_{k-1},w_k)$ be 
$$\xi(z_{k-1},w_k)=[(x_{k-1}+{\nu_{1,k}})^\top\quad (y_{k-1}+{\nu_{2,k}})^\top]^\top \quad \text{when} \quad ||z_{k-1}-z^*||>r,$$
and,
$$\xi(z_{k-1},w_k)=[((1-\lambda)x_{k-1}+{\nu_{1,k}})^\top\quad ((1-\lambda)y_{k-1}+{\nu_{2,k}})^\top]^\top \quad \text{when} \quad ||z_{k-1}-z^*||\leq r,$$
where $0<\lambda<1$, ${\nu_{1,k}}\sim N(0,\sigma^2 I_d)$, ${\nu_{2,k}}\sim N(0,\sigma^2 I_d)$, ${\nu_{1,k}}$ and ${\nu_{2,k}}$ are independent of each other and filtration $\mathcal{F}_{k-1}$, and $\{\nu_{1,k}\}_k$ and $\{\nu_{2,k}\}_k$ are i.i.d sequence. 

Then the problem still remains strongly convex strongly concave in $\mathcal{N}$ but globally it is a convex-concave objective. So, when initiated outside the arbitrarily small $\mathcal{N}$, SGDA faces the same problem as shown in the example in the global response, i.e., when $||z_0-z^*||>r$, one still has, 
\begin{align*}
    E[\|x_k\|_2^2+\|y_k\|_2^2|\mathcal{F}_{k-1}]=(1+\eta_k^2)(\|x_{k-1}\|_2^2+\|y_{k-1}\|_2^2)+2d\eta_k^2\sigma^2
\end{align*}
This clearly shows the problem with SGDA dynamics. We will restate Assumption 4.1 and include this example in the revised version.  

\textbf{**Third response**}

\textbf{**And in the new example the authors provided, there is also a $\lambda$. Does there exist some relationship between the two $\lambda$ s?}

There is no relation between the two $\lambda$. We apologize for the confusion. 

\textbf{**I'm still a little confused about the Verification of Condition 1 of Assumption 6.1 in the Global Response.**}

For a fixed $z$, Condition 1 of Assumption 6.1 is the classical drift condition for Markov chain. Intuitively, for a given $z$. it implies the geometric ergodicity of the chain. Recall that in our global response, for a fixed $z$, the noise $\xi(z,w\_k)$ is given by $z+\nu\_k$ where $\nu\_k=[\nu\_{1,k}^T\quad \nu\_{1,k}^T]^T$ which is an i.i.d noise sequence automatically satisfying the drift condition. The details are below.

Recall that $\mathcal{V}(\nu)=1+||\nu||\_2^2$. Since for Gaussian distribution, all the moments exist, any $\alpha\_0>2$ can be chosen. Set $\alpha\_0=3$. For i.i.d sequence, the conditional distribution of $\nu\_{k+1}$ given $\mathcal{F}\_k$ is still $N(0,\sigma^2 I\_d)$. Then, $$P\_z^l\mathcal{V}^{\alpha\_{0}}(\nu)= P\_z\mathcal{V}^{\alpha\_{0}}(\nu) = E[\mathcal{V}^{\alpha\_{0}}(\nu')]=E[(1+||\nu'||\_2^2)^3]=R\_1,$$
$$P\_z^l(\nu,A)=\mathbb{P}(\nu'\in A)$$,
where $\nu'\sim N(0,\sigma^2 I\_d)$, and $R\_1>1$ is a constant. Choose $$b=(3R\_1-1)/2, \quad \lambda =0.5, \quad \kappa=R\_1,\quad \delta=0.5,$$ and,
$$\mathcal{C}\_1=\{\nu| \mathcal{V}(\nu)\leq (3R\_1)^{1/3}\}$$
$v$ to be the Gaussian measure with mean 0 and covariance $\sigma^2 I\_d$. Then, using $\mathcal{V}(\nu)\geq 1$, 

when $\nu\in\mathcal{C}\_1$,
$$\lambda \mathcal{V}^{3}(\nu)+bI(\nu\in\mathcal{C}\_1)\geq \lambda + b=3R\_1/2>R\_1= P\_z^l\mathcal{V}^{3}(\nu),$$
and when $\nu\notin\mathcal{C}\_1$,
$$\lambda \mathcal{V}^3(\nu)+bI(\nu\in\mathcal{C}\_1)\geq 3\lambda R\_1 =3R\_1/2>R\_1= P\_z^l\mathcal{V}^{3}(\nu),$$
$$P\_z\mathcal{V}^{3}(\nu)=R\_1\leq \kappa \mathcal{V}^{3}(\nu),$$
$$P\_z^l(\nu,A)=v(A)\geq 0.5v(A).$$

\textbf{**Fourth Response**}

That's a great question. We explain below why there is no contradiction.

We argued that for a fixed $z$, the conditional distribution of $\nu\_k$ is independent of the past. But note that \textbf{**the gradient noise is given by $\xi=z+\nu\_k$ that depends on both $z$ and $\nu\_k$. As you point out, for a given $z$, the distribution of the gradient-noise $\xi(z,w\_k)$ is indeed Gaussian but note that the mean of the stationary distribution depends on z.** }

\textbf{**Presumably, our example was confusing because of stating $H(z)=[(y\_k+x\_k)^\top (y\_k-x\_k)^\top]$ at the beginning. That $H(z)$ was just for the given function $f(x,y)$ in the absence of noise.**}

\textbf{**It might help to view $H(z)$ as $E\_{w\sim{\pi\_z}}[H(z,w)]$, i.e., $H(z)$ is not a fixed function of $z$ but keeps changing throughout the dynamics of SEG. Indeed, this is how we introduced our problem in Section 6 (line 200 - 207). This view helps to see that there is no contradiction in the Poisson equation in line 233.**} If one takes expectation on both sides of Poisson equation w.r.t the stationary distribution $\pi\_z$, the left-hand side will be 0 as you point out and the right-hand side will be $E\_{w\sim{\pi\_z}}[H(z,w)]-H(z)=0$ as well. 

We apologize for the confusion about the definition of $H(z)$ and $f(x,y)$. Indeed, trying to optimize a *moving target* is the main challenge with state-dependent Makrovian dynamics. It might be helpful to keep the example in mind discussed in Section 3 . At each time point, on learning the pricing scheme of A and B, the demand distribution changes. So, SEG needs to search for the saddle point of the new expected objective $E[F(\theta,\mu,w)]$ where the data distribution is w.r.t to the new demand distribution. Since SEG does not have access to samples from the stationary distribution, it operates on a state-dependent Markovian sample. This dynamics continues until SEG finds $(\theta^*,\mu^*)$ which is the saddle point of $E\_{w\sim\pi\_{\theta^*,\mu^*}}[F(\theta^*,\mu^*,w)]$. This point is analogous to the notion of *performatively stable* or *equilibirum point* in strategic classification literature. 

We restate our example after changing the presentation. 

Let the state-dependent noise $H(z\_{k-1},w\_k)$ be 
$$H(z\_{k-1},w\_k)=[(y\_{k-1}-{\nu\_{1,k}})^\top\quad (-x\_{k-1}-{\nu\_{2,k}})^\top]^\top \quad \text{when} \quad ||z\_{k-1}-z^*||>r,$$
and,
$$H(z\_{k-1},w\_k)=[(y\_{k-1}+\lambda\_1 x\_{k-1}-{\nu\_{1,k}})^\top\quad (-\lambda\_1 y\_{k-1}-x\_{k-1}-\nu\_{2,k})^\top]^\top \quad \text{when} \quad ||z\_{k-1}-z^*||\leq r,$$
where $0<\lambda\_1<1$, ${\nu\_{1,k}}\sim N(0,\sigma^2 I\_d)$, ${\nu\_{2,k}}\sim N(0,\sigma^2 I\_d)$, ${\nu\_{1,k}}$ and ${\nu\_{2,k}}$ are independent of each other and filtration $\mathcal{F}\_{k-1}$, and $\{\nu\_{1,k}\}\_k$ and $\{\nu\_{2,k}\}\_k$ are i.i.d sequence, and $r>0$ is arbitrarily small. $H(z)=E\_{w\sim{\pi\_z}}[H(z,w)]$. Note that this is the same noisy gradient sequence on which the SEG converged unlike SGDA, i.e., when initiated outside $||z\_{k-1}-z^*||\leq r$ ball, one still has, 
\begin{align*}
    E[\|x\_k\|\_2^2+\|y\_k\|\_2^2|\mathcal{F}\_{k-1}]=(1+\eta\_k^2)(\|x\_{k-1}\|\_2^2+\|y\_{k-1}\|\_2^2)+2d\eta\_k^2\sigma^2
\end{align*}

\iffalse
Then $H(z_k)=[(y_k+x_k)^\top\quad (y_k-x_k)^\top]^\top$. Let the state-dependent noise in $H(z_{k-1},w_k)$ be 
$$\xi(z_{k-1},w_k)=[(x_{k-1}+{\nu_{1,k}})^\top\quad (y_{k-1}+{\nu_{2,k}})^\top]^\top \quad \text{when} \quad ||z_{k-1}-z^*||>r,$$
and,
$$\xi(z_{k-1},w_k)=[((1-\lambda)x_{k-1}+{\nu_{1,k}})^\top\quad ((1-\lambda)y_{k-1}+{\nu_{2,k}})^\top]^\top \quad \text{when} \quad ||z_{k-1}-z^*||\leq r,$$
where $0<\lambda<1$, ${\nu_{1,k}}\sim N(0,\sigma^2 I_d)$, ${\nu_{2,k}}\sim N(0,\sigma^2 I_d)$, ${\nu_{1,k}}$ and ${\nu_{2,k}}$ are independent of each other and filtration $\mathcal{F}_{k-1}$, and $\{\nu_{1,k}\}_k$ and $\{\nu_{2,k}\}_k$ are i.i.d sequence. 
\fi




\textbf{Reviewer aivD}

\textbf{The authors do not show rates of convergence for the proposed algorithms.}

We do show the rate of convergence. Asymptotic $1/\sqrt{n}$ rate is shown in both the noise settings in Theorem 5.2, and Theorem 6.3. If you mean the rate of convergence in expectation, we prove those in equation (25) for the martingale-difference noise, and just above equation (60) in the state-dependent noise case as a part of the proofs for the CLT results. In both cases the rate is $E[\|z_k-z^*\|_2^2]=O(\eta_k)=O(k^{-a})$, $1/2<a<1$. 


\textbf{They also consider that the noise is shared between the two steps of Stochastic Extra Gradient. I do not think this is a very reasonable assumption, since the second update of the algorithm, requires the calculation of the first update. }

Note that using the same sample to evaluate the updates of SEG is possible in most machine learning applications like bi-linear games, generative adversarial networks, and adversarial training [1]. In fact there are examples where the SEG iteration persistently diverges when using independent samples [1]. Intuitively, this happens because with independent samples, SEG is no longer an approximation of proximal point method and hence can diverge. For detailed explanation see [Sec. 1 of 1, Sec. 2 of 2, Sec. 1.1 of 3]. 

\textbf{How do we know that the Markov Chain has a stationary distribution (line 204)?}

Under Condition 1, Assumption 6.1 (which is classical drift condition), for any fixed $z$, the Markov chain will have a stationary distribution. We admit this needs to be clarified in the beginning of Section 4. We will update the final version accordingly. 

\textbf{How exactly are the sets are defined?}

One example would be take balls of increasing radii. 

\textbf{Could the authors explain why the truncation is necessary? Specifically, in Lemma 6.1, which is the component of the noise that cannot be controlled but when considering truncated sets it can?}

**In Lemma 6.1, the components $\nu_k$ and $\zeta_k$ can diverge unless the dynamics are contained in a compact set.** State-dependent Markovian noise allows for adversarial setting, for example multi-task strategic classification problems. In such problems, the dependence of the transition kernel on the state $z_k$ allows for adversarial noise sequence such that the iterates are pushed away from $z^*$. 

**Intuitively, truncation and reinitialization with a larger compact set allows the algorithm to run long-enough such that the drift towards $z^*$ dominates over the stepsize-modulated noise component while the iterates remain contained in that compact set. In fact, the proof of Claim 6.1 depends on this observation. This concept is captured in the definition of $\mathcal{A}$ in eq. (49) where $S_{l,n}$ (defined in (48)) is the step-size modulated noise component.**

Minor: We will fix the typos. 

[1] Li, Chris Junchi, Yaodong Yu, Nicolas Loizou, Gauthier Gidel, Yi Ma, Nicolas Le Roux, and Michael Jordan. "On the convergence of stochastic extragradient for bilinear games using restarted iteration averaging." In International Conference on Artificial Intelligence and Statistics, pp. 9793-9826. PMLR, 2022.

[2] Mishchenko, Konstantin, Dmitry Kovalev, Egor Shulgin, Peter Richtárik, and Yura Malitsky. "Revisiting stochastic extragradient." In International Conference on Artificial Intelligence and Statistics, pp. 4573-4582. PMLR, 2020.

[3] Gorbunov, Eduard, Hugo Berard, Gauthier Gidel, and Nicolas Loizou. "Stochastic extragradient: General analysis and improved rates." In International Conference on Artificial Intelligence and Statistics, pp. 7865-7901. PMLR, 2022.

\textbf{Reviewer i4sG}

\textbf{``The assumption that at each iteration the noise sample is shared between the two iterates could be limiting in a few scenarios. In practice, in numerous settings, this is a reasonable assumption (accessing twice the same sample) but the authors may want to emphasize such potential limitation. "}

Note that using the same sample to evaluate the updates of SEG is possible in most machine learning applications like bi-linear games, generative adversarial networks, and adversarial training [1]. In fact there are examples where the SEG iteration persistently diverges when using independent samples [1]. Intuitively, this happens because with independent samples, SEG is no longer an approximation of proximal point method and hence can diverge. For detailed explanation see [Sec. 1 of 1, Sec. 2 of 2, Sec. 1.1 of 3]. 

We will clarify this in the final version. 

\textbf{Q1. ``In the experiments, what do you mean by "hypothetical strongly convex strongly concave"?}

1. This is to mean that unlike the case where $A_1,B_1,A_2,B_2,\rho$ are nonzero, which corresponds to the example presented in Section 3, the case $A_1=B_1=A_2=B_2=\rho=0$ does not correspond to the real-life example in Section 3 but still is a strongly convex strongly concave Saddle Point Problem with martingale-difference noise. We will rewrite the sentence and clarify it. 


**Numerous saddle point problems are simply convex concave. Additional squared regularization... surrogate problem with respect to the original problem?**

Squared regularization can be added to a convex-concave problem to achieve different goals. For example, in a convex-concave game, a squared regularizer favors a Nash equilibrium where the cost of a playing strategy increases with the absolute value of the strategy. In the saddle-point formulation of a linear regression problem, an $L_2$ regularizer is added to identify sparse solution [Section 6 of 4]. Our result quantifies the asymptotic randomness of the averaged iterate of the SEG algorithm around these saddle points.

If there is no such reason like above to introduce a regularizer, one can introduce an arbitrarily small but positive squared regularizer to turn the problem into strongly convex strongly-concave. Then one can use our results to characterize the asymptotic randomness of SEG around the saddle point of this perturbed problem that is arbitrarily close to the original convex-concave problem for small regularizer (by smoothness of $f(x,y)$). In the special case where the saddle-point is at $(0,0)$, the squared regularizer does not change the saddle point at all. 

%This small regularizer perturbs the saddle point of the original convex-concave problem only by a small amount (by smoothness of $f(x,y)$).

\textbf{``If I understood correctly a set of balls with geometrically increasing radii could work for example."} 

That is correct. We will mention it explicitly in the paper. 

Minor details:
We will fix the writing and make other necessary changes. 



[1] Li, Chris Junchi, Yaodong Yu, Nicolas Loizou, Gauthier Gidel, Yi Ma, Nicolas Le Roux, and Michael Jordan. "On the convergence of stochastic extragradient for bilinear games using restarted iteration averaging." In International Conference on Artificial Intelligence and Statistics, pp. 9793-9826. PMLR, 2022.

[2] Mishchenko, Konstantin, Dmitry Kovalev, Egor Shulgin, Peter Richtárik, and Yura Malitsky. "Revisiting stochastic extragradient." In International Conference on Artificial Intelligence and Statistics, pp. 4573-4582. PMLR, 2020.

[3] Gorbunov, Eduard, Hugo Berard, Gauthier Gidel, and Nicolas Loizou. "Stochastic extragradient: General analysis and improved rates." In International Conference on Artificial Intelligence and Statistics, pp. 7865-7901. PMLR, 2022.

[4] Aryan Mokhtari, Asuman Ozdaglar, and Sarath Pattathil. A unified analysis of extra-gradient and optimistic gradient methods for saddle point problems: Proximal point approach. In International Conference on Artificial Intelligence and Statistics, pages 1497–1507. PMLR, 2020. http://proceedings.mlr.press/v108/mokhtari20a/mokhtari20a.pdf

\textbf{Reviewer FbMP}

\textbf{``I do have a question. Can the techniques in this work be used to understand the stability of saddle points of SGD? For example, do the authors think that the techniques used in this work can be related to the problem studied in https://arxiv.org/abs/2107.11774?"}

In the cited paper, the goal of the dynamics is to escape the saddle points since one is interested in the minima. In contrast, we are interested to find the saddle point. So these two papers have different goals. 

Although, extension of our results to the non-aymtptotic regime, to capture the uncertainty of SGD with constant learning rate, will be quite interesting to explore.  

\newpage
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{xn2yn2diverge.png}
    \caption{We plot $\|\sqrt{n}\bar{x}_n\|_2^2+\|\sqrt{n}\bar{y}_n\|_2^2$ over iterations to compare SEG with SGDA. The objective function is $f(x,y)=x^\top y+0.5 \|x\|_2^2-0.5 \|y\|_2^2$. The state-dependent noise setup is as described in the global response. Here we choose $\sigma=0.01$. Even with this small noise variance the difference of performance between SGDA and SEG is quite clear.}
    \label{fig:segsgda}
\end{figure}
\clearpage 

==> reproducibility.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. Yes
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. Yes
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. Not Applicable
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. Yes
   \item Complete proofs of all theoretical results. Yes
   \item Clear explanations of any assumptions. Yes
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). Yes
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). Yes
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). Yes
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). Not Applicable
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. Not Applicable
   \item The license information of the assets, if applicable. Not Applicable
   \item New assets either in the supplemental material or as a URL, if applicable. Not Applicable
   \item Information about consent from data providers/curators. Not Applicable
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. Not Applicable
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. Not Applicable
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. Not Applicable
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. Not Applicable
 \end{enumerate}

 \end{enumerate}

